Scaling Robot Supervision to Hundreds of Hours with RoboTurk: Robotic Manipulation Dataset through Human Reasoning and Dexterity

Large, richly annotated datasets have accelerated progress in fields such as computer vision and natural language processing, but replicating these successes in robotics has been challenging. While prior data collection methodologies such as self-supervision have resulted in large datasets, the data can have poor signal-to-noise ratio. By contrast, previous efforts to collect task demonstrations with humans provide better quality data, but they cannot reach the same data magnitude. Furthermore, neither approach places guarantees on the diversity of the data collected, in terms of solution strategies. In this work, we leverage and extend the RoboTurk platform to scale up data collection for robotic manipulation using remote teleoperation. The primary motivation for our platform is two-fold: (1) to address the shortcomings of prior work and increase the total quantity of manipulation data collected through human supervision by an order of magnitude without sacrificing the quality of the data and (2) to collect data on challenging manipulation tasks across several operators and observe a diverse set of emergent behaviors and solutions. We collected over 111 hours of robot manipulation data across 54 users and 3 challenging manipulation tasks in 1 week, resulting in the largest robot dataset collected via remote teleoperation. We evaluate the quality of our platform, the diversity of demonstrations in our dataset, and the utility of our dataset via quantitative and qualitative analysis. For additional results, supplementary videos, and to download our dataset, visit http://roboturk.stanford.edu/realrobotdataset .

==> 1_intro.tex <==
\section{INTRODUCTION}

%data helps in learning. 

%but robotics has a data problem because data needs demonstrations not labelling.

% others have collected data through self supervision. 

% but this is low-signal to noise. For complex tasks, focused demonstration is needed. Others (deep imitation paper) used demonstrations showcase that data can be useful for fixed tasks. 

% However, the requirements of data increase when task complexity and variability grows. 

% Crowdsourcing can help in filling this need. 

% This paper presents an approach to collect 100+ hours of data on real robots. we extend the roboturk framework presented in []. the key challenges are...

% summary of contributions


% P1: Large datasets are useful.

Crowdsourcing mechanisms such as Amazon Mechanical Turk have facilitated the creation of large, richly annotated datasets. The advent of datasets, sizing in millions, has accelerated progress in computer vision and natural language processing~\cite{deng2009imagenet,rajpurkar2018squad2} by enabling for the development and evaluation of a wide set of learning algorithms. Efforts to aggregate similarly large amounts of data have taken place in the field of robot manipulation.

% P2: There have been prior efforts to collect datasets for robotics. 
Prior work has leveraged online self-supervised data collection ~\cite{levine2016learning, pinto2016supersizing} and off-policy reinforcement learning ~\cite{kalashnikov2018qt} to collect large quantities of physical robot data for tasks such as grasping. However, data collected in this manner suffers from some major drawbacks. The data can have a low signal-to-noise ratio, since a large portion of the data is collected by applying random robot controls. Correspondingly, the time it takes to start collecting high-quality data can be prohibitively large in turn limiting the task complexity. 

In addition, these methods require a loss or reward function that can be evaluated by the robot from available information (for example, a successful grasp), but complex tasks often lack straightforward signals that can be used for this purpose. Loss or reward signals could also require careful engineering. By contrast, collecting task demonstrations from humans replaces the need for a self-supervised loss or reward with a set of demonstrations of successful task executions.

Prior work ~\cite{zhang2017deep} has shown that collecting task demonstrations from humans and applying Imitation Learning ~\cite{argall2009survey,pomerleau1989alvinn} can achieve success on a set of restricted task instances. Although the data collected has a higher signal-to-noise ratio due to the human in the loop, these approaches have been limited in both the scale of data collected and the complexity of the tasks used for data collection. The ideal data collection approach would be able to collect quantities of data similar to self-supervised approaches while maintaining the quality of data that is collected through human supervision and control. 

We further emphasize that neither approach places guarantees on the \textit{diversity} of the data collected. However, humans can potentially demonstrate several interesting strategies that vary across people, and across situations. This is where the notion of crowdsourcing large datasets could really benefit data collection in robotics.

Replicating the success and impact that large-scale datasets have had in other fields for robotics has been challenging. Since robotic motion is physical and occurs in real-time, annotations for complex manipulation tasks must occur in \textit{real-time}. In other words, the expert needs to \textit{demonstrate} how to perform a task in real-time, instead of just labelling data in an offline setting. In order to provide task demonstrations, a user needs to interact with a physical robot in real-time. Robotic teleoperation provides a natural mechanism for this.

\ajay{some brief overview of teleoperation}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/pull_figure_v1.png}
    \caption{Pull figure. 3 people in thought bubbles in different viewpoints and 3 robots.}
    \label{fig:intro}
\end{figure}

% Key question: how to collect large set of _diverse_ task demonstrations on physical robots? Several challenges such as safety, system design, lag for real-time video, depth perception, varied instances and tasks for human reasoning, and an interface that actually puts the human in the driver seat, allowing for fluid, natural control and full expression of how the robot arm should move. This is like kinesthetic teaching at a distance, grab end effector and move it around. 

Enabling several remote users to each control a separate physical robot arm is challenging due to the need for a tightly coupled user-robot real-time control loop that is robust to stochastic delays in both robot motor actuation and network speeds.

Given the constraints that collecting data on physical robotic platforms imposes, one might wonder why large-scale datasets collected in simulators are not preferred. While collecting data from simulators is certainly easier and can provide more detailed ground-truth information, the differences between simulated data and actual physical data are substantial, Indeed, simulation to real world transfer is a major open problem in the field. Furthermore, while there have been impressive strides recently in the fidelity of physical simulators, there are certain classes of objects and material properties that remain difficult to simulate in real-time, such as soft bodies, liquids, and objects with non-standard shapes, while the physical world places no such limitations. This underscores the importance of collecting high-quality data directly on physical hardware.

To that end, we propose an approach to collect task demonstrations on physical robots from humans to scale data collection along two dimensions: the quantity of data collected, and the diversity of data collected. To tackle this challenge, we extended the RoboTurk platform \cite{mandlekar2018roboturk} to enable scalable data collection on physical robot arms. Extending RoboTurk to collect data on real robot arms introduces a number of challenges as compared to collecting data in simulation. The original RoboTurk platform allowed for crowdsourcing demonstrations in simulated robot domains quickly by collecting data across several simultaneous users. By contrast, physical robot data collection is bottlenecked by the number of actual robot arms available for data collection. Furthermore, teleoperating a physical robot remotely over a network introduces additional delays due to robot hardware limits in actuation and control of the arm, as compared to robots in simulation. In addition, careful safety measures must be taken to prevent remote users from damaging the robot arms. Finally, the data collection mechanism must deal with data streams coming from different sensors at different rates. Our extension to the RoboTurk platform solves each of these challenges. 

% Solving this challenge requires providing a natural control interface for humans to control robots, a high-quality real-time perceptual feedback loop for the human operator, and safety mechanisms for the robots. 

We present a large-scale diverse dataset collected using RoboTurk on 3 physical Sawyer robot arms. The dataset contains over 110 hours of manipulation data collected by 54 users across 3 complex manipulation tasks, each of which requires dexterous manipulation coupled with cognitive reasoning. This is the largest dataset ever collected by humans via robot teleoperation. 

% Hypothesis: dataset is the first of its kind - large-scale dataset which captures human knowledge coupled to low-level robot control, together. Only possible with a system like RoboTurk. 

% Goal of system: Endow generalizable robots with human knowledge. We present this dataset collected with the system to take a first step in this direction.

\noindent \textbf{Summary of Contributions}:
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    partopsep=1ex,
    parsep=1ex,
    leftmargin=*,
    itemindent=3ex
    ]
\item We extend RoboTurk, a data collection platform that allows remote workers to collect task demonstrations using a smart phone as a motion controller, to enable data collection on physical robot arms. Our new platform accounts for limited robot resources, additional delays introduced by robot hardware, the need for safety measures to protect the robots from harm, and data collection from multiple sensor streams at different rates. The platform allows for collecting large amounts of physical robot manipulation data through diverse sets of remote users. 
\item We present the largest robot dataset collected via remote teloperation. Over the course of 1 week, we collected over 110 hours of data across 54 users and 3 challenging manipulation tasks: Object Search, Tower Creation, and Laundry Layout.
\item We evaluate the quality of our platform, the diversity of demonstrations in our dataset, and the utility of our dataset via quantitative and qualitative analysis.
\end{enumerate}
